Squeezed light from a levitated nanoparticle at room temperature

Quantum measurements of mechanical systems can produce optical squeezing via ponderomotive forces. Its observation requires high environmental isolation and efficient detection, typically achieved by using optical cavities and cryogenic cooling. Here we realize these conditions by measuring the position of an optically levitated nanoparticle at room temperature and without the overhead of an optical cavity. We use a fast heterodyne detection to reconstruct simultaneously orthogonal optical quadratures, and observe a noise reduction of $9\%\pm0.5\%$ below shot noise. Our experiment offers a novel, cavity-less platform for squeezed-light enhanced sensing. At the same time it delineates a clear and simple strategy towards observation of stationary optomechanical entanglement.

==> oldintros.tex <==

Squezing of light history, chi2 4wave mixing \cite{Slusher1985}, PDC\cite{Wu1986}, kerr in fiber\cite{Shelby1986}. Record 15dB \cite{Vahlbruch2016} 
Why is ponderomotive squeezing interesting? because its such a simple concept: quantum fluctuations... bla bla..
History of ponderomotive squeezing.. 


\textit{We need a pitch -- I’ll think about it.} 
Quantum fluctuations of the radiation pressure force imparted on a mechanical oscillator coupling to a light field disturbs its motion. Consequently, the mechanical oscillator is driven by these intrinsic fluctuations in the light field, giving rise to an intensity-dependent non-linear force on the oscillator. 

Quantum fluctuations of the radiation pressure force on a mechanical oscillator coupling to a light field disturbs its motion. Consequently, the mechanical oscillator is driven by these intrinsic fluctuations in the light field, giving rise to an intensity-dependent non-linear force on the oscillator
The motion of the oscillator is imprinted on the phase of the light which interacted with the oscillator, thus creating correlations between the phase and amplitude of the light field. 

Coupling of the mechanical oscillator to a thermal environment spoils this effect. This limitation is commonly surpassed by enhancing the optomechanical interaction with optical cavity, and reducing the temperature of the environment in a cryostat. In this work we demonstrate optomechanical squeezing of light at room temperature, and without a cavity.     


This phenomenon, coined ponderomotive squeezing, is a prime example of a quantum effect involving potentially macroscopic mechanical oscillators. , Fabre \textit{et al.}  \cite{fabre1994ponderomotive} and Mancini and Tombesi \cite{mancini1994ponderomotive} pointed out the potential of a suspended mirror in an optical cavity to generate squeezed light.
, even in presence of thermal fluctuations which also disturb the motion of the mechanical oscillator. Building on these studies, this optomechanical cavity was suggested to generate non-classical states of light ~\cite{mancini1997, bose1997ponderomotive} and of the mirror \cite{bose1997ponderomotive}, and proposed as a solution for noise reduction in gravitational wave detectors \cite{corbitt2006ponderomotive}.


Correlations between the radiation pressure and the position of a mechanical oscillator were first observed by Marino \textit{et al.}~\cite{Marino2010} and Verlot \textit{et al.}~\cite{Verlot2010} using an input field with increased amplitude noise with respect to the vacuum state in order to amplify the correlation term. Noise reduction below the quantum limit using this mechanism was first achieved with an ensemble of cold atoms in a cavity~\cite{Brooks2012} and thereafter in solid-state cavity-optomechanical systems in cryogenic environment ~\cite{SafaviNaeini2013,Purdy2013, Sudhir2017,Ockeloen2018, Mason2019}. At room temperature noise reduction was demonstrated with solid state mechanical systems~\cite{Purdy2017, Sudhir2017rt} and with the 40-kg mirrors used in LIGO~\cite{Yu2020}, while squeezing of light was recently achieved~\cite{Aggarwal2020}, with a movable mirror in an optical cavity. 

We levitate a nanoparticle in a tightly-focussed tweezer %
In essence, the effect leading to ponderomotive squeezing in the absence of a cavity is comparable to what happens with a cavity. Nonetheless, in the following we detail the derivation and stress the main differences with the cavity-based platforms. We then present experimental data demonstrating unambiguous squeezing of a given output optical field quadrature as well as excellent agreement with our theoretical description.

##### lORENZO WORKING IN THIS SECTION####


\section*{Theory}

The state of the light field after the optomechanical interaction can be derived by integrating the equations of motion of the output field creation and annihilation operators $\cdag$ ad $\cop$ in the Heisenberg picture\cite{supplementary}. Any arbitrary optical quadrature can then be expressed in terms of linear combination of the two orthogonal quadratures reconstructed from the demodulation of the heterodyne measurement:

The complete optical Next, we briefly discuss the calibration of our measurements and the determination of all relevant physical parameters: thermal occupation ($n$), decoherence rates ($\Gamma_{ba}$ and $\Gamma_{th}$), and detection efficiency $\eta_d$.
A rigorous determination of these parameters from the measured spectra is not straightforward, and details are provided in the Supplementary Information \cite{}.
First, we once again employ the heterodyne measurement \textcolor{OliveGreen}{to compute and analyze} \st{to analyze} the cross correlation spectra \textcolor{OliveGreen}{ \st{$S_{0,\frac{\pi}{2}}$} and} $S_{\frac{\pi}{4},\frac{3\pi}{4}}$, \textcolor{OliveGreen}{as this contains the thermal motion contribution and does not required detailed knowledge of the mechanical parameters,} for a calibration-free estimate of the average occupation\cite{Purdy2017}, \blue{see Supplementary Information}. With an estimated thermal decoherence rate of $\Gamma_\mathrm{th}/2\pi=2.7\,\mathrm{kHz}$  at $1.5\times 10^{-8}$\,$\mathrm{mbar}$, absolute thermometry leads to the measurement induced backaction decoherence $\Gamma_\mathrm{ba}/2\pi=4.9\,\mathrm{kHz}$. The deduced quantum cooperativity is $C_\mathrm{q}=\Gamma_\mathrm{ba}/\Gamma_\mathrm{th} = 1.8$, in good agreement with our expectations~\cite{magrini2021}.
Having independently determined the decoherence rates, we can finally fit \eqref{eq:ponderomotive1} to the autocorrelation quadrature spectra at all angles, with only 2 strongly uncorrelated free parameters: $\eta_d$ and $\Omega_z$. The fits result in a detection efficiency (per quadrature) of $\eta_d = 0.12$. These values were used to compute the expected spectrum at the optimal squeezing angle shown in Fig.\ref{fig:2}.

The measured squeezing is slightly smaller than expected in our experimental conditions. Indeed, at the optimal quadrature angle, the strongest squeezing is expected in a very narrow band very close to resonance. Here, the small frequency fluctuations due to mechanical drifts in our setup are enough to wash out this narrow feature at the optimal angle\cite{supplementary}. At larger angles the squeezing is distributed over a broader band, and further away from resonance, as shown in the full squeezing spectrogram represented figure \ref{fig:3}.






Although the observed squeezing is moderate, and even in perspective, optomechanical systems are far from being competitive with the conventional methods of squeezed light generation~\cite{Andersen2016, Vahlbruch2016}, this result represents a crucial step towards the observation of entanglement between the light and the mechanical motion of a macroscopic oscillator.




Prominent examples include searches for gravitational waves [Abb+16], as well as for signatures of physics beyond the current standard model such as dark
matter, dark energy [MRG14; Car+20; MG21; GPK10; Ham+15; Ove+18; Lee+20],
quantum gravity [Pik+12; Baw+15; Bel+16] and even string theory [Ger+08; Lee+20;
Tan+20]. 

In this context optical levitation represents one of the most promising experimental methods. The advantage of optically levitated systems is that light, and only light, defines all of the relevant experimental parameters. It
defines not only the measurement process and quantum decoherence rates, but also
the function of the potential landscape in which the mechanical object lives. The result is an extremely versatile quantum system, which evolves in time according to a Hamiltonian that can be dynamically tuned in almost all of its degrees of freedom. Experiments... in the classical regime   andf Recently enterd the quqntum regime with demonstationof ground state cooling.   

\textcolor{blue}{Extracting information from a quantum system typically comes at a cost, the measurement back-action. Consider a dielectric nanoparticle levitating in a tweezer. Position information is gained from the photons scattered by the particle. However, the tweezer light contains intrinsic photon number fluctuations, in turn exciting the particle's motion. Position fluctuations of the nanoparticle are then transduced to the phase of the output field, leading to correlations between the phase and amplitude quadratures of the detected light. For a certain angle of the detected quadratures, the output light becomes squeezed.  Inspired by the formal analogy with the optical Kerr effect, this phenomenon, coined ponderomotive squeezing, was first introduced by Fabre \textit{et al.}  \cite{fabre1994ponderomotive} and Mancini and Tombesi \cite{mancini1994ponderomotive}, by proposing to use a suspended mirror in an optical cavity to generate squeezed light.}\\
\textcolor{blue}{In practice, the measurement back-action is not the only disturbance at play. Environmental thermal fluctuations also excite the motion of the particle. To observe squeezing, the back-action noise should dominate. Thus, experiments demonstrating ponderomotive squeezing have relied on optical cavities~\cite{Brooks2012,Purdy2017, Sudhir2017rt,Yu2020,Aggarwal2020} to enhance the strength of the measurement, and on cryogenics~\cite{Marino2010, Verlot2010,SafaviNaeini2013,Purdy2013, Sudhir2017,Ockeloen2018, Mason2019} to reduce the thermal noise contribution.\\
Here, we demonstrate ponderomotive squeezing at room temperature and without an optical cavity, as a modern adaptation of Heisenberg's microscope, a thought experiment where he envisioned the optical position measurement of an electron and the inevitable measurement back-action. Our measurement scheme relies on heterodyne detection and a subsequent demodulation to access two orthogonal quadratures of the field after its interaction with the particle. By varying the demodulation phase, full state tomography is performed, making this technique a powerful tool for future experiments involving quantum effects with levitated nanoparticles.}

     


\textcolor{OliveGreen}{The mere act of observing and acquiring information disturbs the state of a system. This fundamental and inevitable phenomenon find in nature was… maybe?} The act of observation disturbs the state of a system. This fundamental property of quantum mechanics was elegantly formulated in the famous Gedankenexperiment known as the ``Heisenberg microscope''~\cite{heisenberg1927}, where light is used to measure the position of an electron. Similarly, the measurement of the position of a dielectric nanoparticle levitating in an optical tweezer will result in a measurement backaction.
where light is used to measure the position of an electron. As a consequence the momentum of the electron is disturbed by the intrinsic fluctuations in the light field, giving rise to an intensity-dependent non-linear radiation pressure force, a measurement backaction.
\textcolor{Blue}{The random quantum fluctuations in the photon number of the optical field results in a fluctuating} force noise driving the motion of the measured object. While the interaction leaves the optical amplitude unchanged, position fluctuations of the nanoparticle are transduced to the phase of the output field. Given that the force noise scales with the amplitude of the incoming field, this optomechanical interaction leads to correlations between the outgoing amplitude and phase \textcolor{Blue}{light} quadratures.
The input noise fluctuations are vacuum-limited, since the measured object is interacting with a coherent light state. Consequently, these correlations can result, for some linear combination of amplitude and phase, in a reduction of the total noise of the field quadrature below the shot noise level, leading to a squeezed state of light.
Inspired by the formal analogy with the optical Kerr effect, this phenomenon, coined ponderomotive squeezing, was first introduced by Fabre \textit{et al.}  \cite{fabre1994ponderomotive} and Mancini and Tombesi \cite{mancini1994ponderomotive}, by proposing to use a suspended mirror in an optical cavity to generate squeezed light.
Although a semi-classical theory of light and mechanics is enough to describe this effect, its observation requires both exceptional isolation from the environment and a strong measurement interaction.\textcolor{Blue}{\st{, and represents a fundamental benchmark for the observation of quantum effects involving potentially macroscopic mechanical oscillators.}}
The measurement process indeed is not the only disturbance at play. Thermal fluctuations \blue{typically contribute significantly to the drive of small mechanical objects}, burying the quantum correlations introduced by the weak measurement into thermal noise. Thus, experiments demonstrating ponderomotive squeezing have relied on optical cavities~\cite{Brooks2012,Purdy2017, Sudhir2017rt,Yu2020,Aggarwal2020} to enhance the strength of the measurement, and on cryogenics~\cite{Marino2010, Verlot2010,SafaviNaeini2013,Purdy2013, Sudhir2017,Ockeloen2018, Mason2019} to reduce the thermal noise contribution.\\
Here, we demonstrate ponderomotive squeezing at room temperature and without an optical cavity, realizing Heisenberg's Gedankenexperiment in its simplest form. \textcolor{Blue}{Our measurement scheme relies on heterodyne detection and a subsequent demodulation to access two orthogonal quadratures of the field after its interaction with the particle. By varying the demodulation phase, full state tomography is performed, making this technique a powerful tool for future experiments involving quantum effects with levitated nanoparticles.}

\textcolor{WildStrawberry}{The act of observation disturbs the state of a system. This fundamental property of quantum mechanics was formulated in the famous Gedankenexperiment known as the ``Heisenberg microscope''~\cite{heisenberg1927}, where light is used to measure the position of an electron. The necessary random fluctuations in the photon number define a fluctuating force which drives the motion of the measured object, which is in turn imprinted onto the phase of light emerging from the measurement. As a result, the measurement interaction, protracted in time,  establishes a correlation between the non-commuting observables of light (amplitude and phase), which results in a reduction of the noise of a field quadrature below shot noise: a squeezed state of light. Inspired by the formal analogy with the optical Kerr effect, this phenomenon, coined ponderomotive squeezing, was first introduced by Fabre \textit{et al.}  \cite{fabre1994ponderomotive} and Mancini and Tombesi \cite{mancini1994ponderomotive}, by proposing to use a suspended mirror in an optical cavity to generate squeezed light.
The first experimental observation of correlations betweeen radiation-pressure force noise and the position of a mechanical resonator was achieved by Marino \textit{et al.}~\cite{Marino2010} and Verlot \textit{et al.}~\cite{Verlot2010} using an input field with an increased classical intensity noise in order to amplify the correlation term. Observation of noise reduction by ponderomotive squeezing below shot noise was achieved two years later by Brooks \textit{et al.} using ultracold atoms in an optical cavity \cite{Brooks2012}, and shortly after demonstrated in solid state optomechanical systems in a cryogenic environment~\cite{SafaviNaeini2013,Purdy2013, Sudhir2017,Ockeloen2018, Mason2019}. At room temperature, noise reduction due to the radiation pressure-position correlation was observed~\cite{Purdy2017, Sudhir2017rt}, even on kg-scale objects~\cite{Yu2020}, however the high thermal noise contribution did not allow to obtain squeezed light. Recently the first demonstration of optomechanical ponderomotive squeezing was achieved at room temperature by Aggarwal \textit{et al.}~\cite{Aggarwal2020}, with a movable mirror inside an optical cavity.
Coupling to the environment degrades the squeezing of the detected light, burying the burying the quantum correlations into thermal noise. For this reason experiments demonstrating noise reduction below to date have relied on optical cavities to enhance the strength of the measurement, and on cryogenic cooling to reduce the thermal noise contribution. In this work, we detect light scattered by a nanoparticle  that is optically levitated in ultra-high vacuum, and show ponderomotive squeezing in its simplest form: at room temperature and without an optical cavity. Although the observed squeezing is moderate, and even in perspective, optomechanical systems are far from being competitive with the conventional methods of squeezed light generation~\cite{Andersen2016, Vahlbruch2016}, this result represents a crucial step towards the observation of entanglement between the light and the mechanical motion of a macroscopic oscillator. For this reason, we base our measurement on heterodyne detection, which allows us to recover, at all times, a complete tomography of the optical state.}

